Supervised Domain Adaptation for Recognizing Retinal Diseases from Wide-Field Fundus Images

This paper addresses the emerging task of recognizing multiple retinal diseases from wide-field (WF) and ultra-wide-field (UWF) fundus images. For an effective use of existing large amount of labeled color fundus photo (CFP) data and the relatively small amount of WF and UWF data, we propose a supervised domain adaptation method named Cross-domain Collaborative Learning (CdCL). Inspired by the success of fixed-ratio based mixup in unsupervised domain adaptation, we re-purpose this strategy for the current task. Due to the intrinsic disparity between the field-of-view of CFP and WF/UWF images, a scale bias naturally exists in a mixup sample that the anatomic structure from a CFP image will be considerably larger than its WF/UWF counterpart. The CdCL method resolves the issue by Scale-bias Correction, which employs Transformers for producing scale-invariant features. As demonstrated by extensive experiments on multiple datasets covering both WF and UWF images, the proposed method compares favorably against a number of competitive baselines.

==> table/ablation.tex <==
\begin{table*}[htb]
    \caption{\textbf{The effect of different components.}}
    \label{tab:ablation}
    \centerline{
        \scalebox{1.}{
            \begin{tabular}{c| c| c|l  rr  rr  r}
                \hline
                \textbf{FoV matching} & \textbf{Mix up} & \textbf{Score fusion} && \textbf{RFMiD$\rightarrow$TOP} && \textbf{CFP-MD$\rightarrow$CFP-UWF} && \textbf{CFP-MD$\rightarrow$CFP-WF}  \\
                \cmidrule{1-3} \cmidrule{5-5}  \cmidrule{7-7} \cmidrule{9-9}            
               
                           &            &            && 0.640$\pm$0.018 && 0.623$\pm$0.005 && 0.680$\pm$0.018 \\
                \checkmark &            &            && 0.660$\pm$0.013 && 0.658$\pm$0.007 && 0.684$\pm$0.002 \\
                \checkmark & \checkmark &            && 0.677$\pm$0.032 && 0.662$\pm$0.007 && 0.684$\pm$0.012 \\
                \checkmark & \checkmark & \checkmark && 0.678$\pm$0.032 && 0.675$\pm$0.009 && 0.691$\pm$0.006 \\
                \hline
            \end{tabular}
        }           
    }
\end{table*}

==> table/backbone.tex <==
\begin{table}[htb]
    \caption{\textbf{Performance on }. }
    \label{tab:backbone}
    \renewcommand{\arraystretch}{1}
    \centerline{
        \scalebox{0.5}{
            \begin{tabular}{@{}lrrrrrrrrr@{}}
        \toprule
                \textbf{Method} & \textbf{mAP} & \textbf{DR} &  \textbf{RVO} & \textbf{LP} & \textbf{DM} & \textbf{RD} & \textbf{TF} & \textbf{AMD} & \textbf{MEM}\\
                \midrule
                Training data: UWF-MD
                \texttt{ResNet-50} \\
                \texttt{Inception-V3} \\
                \texttt{EfficientNet-B3} \\
                \texttt{Swin-Transformer tiny} \\
                
                \midrule
                Training data: WF-MD
                \texttt{ResNet-50} \\
                \texttt{Inception-V3} \\
                \texttt{EfficientNet-B3} \\
                \texttt{Swin-Transformer tiny} \\

                \midrule
                Training data: TOP
                \texttt{ResNet-50} \\
                \texttt{Inception-V3} \\
                \texttt{EfficientNet-B3} \\
                \texttt{Swin-Transformer tiny} \\
        \bottomrule
            \end{tabular}
        }           
    }
\end{table}

==> table/fov.tex <==
\begin{table*}[htb]
    \caption{\textbf{Model performances without CFP images.}}
    \label{tab:fov}
    \centerline{
        \scalebox{1.}{
            \begin{tabular}{l l  rr  rr  r r}
                \hline
                \textbf{Model} &&  \textbf{RFMiD$\rightarrow$TOP} && \textbf{CFP-MD$\rightarrow$CFP-UWF} && \textbf{CFP-MD$\rightarrow$CFP-WF}\\
                \cmidrule{1-1} \cmidrule{3-3} \cmidrule{5-5} \cmidrule{7-7}
                
                EfficientNet-B3                && 0.647$\pm$0.036 && 0.622$\pm$0.018 && 0.669$\pm$0.003\\
                EfficientNet-B3 + FoV matching && 0.652$\pm$0.024 && 0.638$\pm$0.010  && 0.661$\pm$0.009\\
                %EfficientNet-B3                & CFP      && 0.658$\pm$0.043 && 0.623$\pm$0.005 && 0.680$\pm$0.018\\
                %EfficientNet-B3 + FoV matching & CFP      && \\
                \hline
            \end{tabular}
        }
    }
\end{table*}

==> table/sota-complete.tex <==
\begin{table*}[htb]
    \caption{\textbf{AP value of different methods.}}
    \label{tab:sota-complete}
    \centerline{
        \scalebox{0.5}{
            \begin{tabular}{l rr  r  r  r  r  r  r  r  r}
                \textbf{Method} && \textbf{Mean} & \textbf{DR} & \textbf{RVO} & \textbf{LP} & \textbf{DM} & \textbf{RD} & \textbf{TF} & \textbf{AMD} & \textbf{MEM} \\
                \cmidrule{1-1} \cmidrule{3-11}
                CFP-MD to WF-MD\\
                \cmidrule{1-1} \cmidrule{3-11}
                Model-CFP   &&          &        &         &          &        &          &        &         &    \\
                Model-UWF   &&          &        &         &          &        &          &        &         &     \\
                Model-Transfer   &&          &        &         &          &        &          &        &         &     \\

                DDC\cite{DDC}   &&          &        &         &          &        &          &        &         &     \\
                DANN\cite{DANN}   &&          &        &         &          &        &          &        &         &       \\
                ADDA\cite{ADDA}   &&          &        &         &          &        &          &        &         &            \\
                MDD\cite{MDD}   &&          &        &         &          &        &          &        &         &            \\
                FixBi\cite{FixBi}   &&          &        &         &          &        &          &        &         &            \\
                CycleGan\cite{FixBi}   &&          &        &         &          &        &          &        &         &           \\
                Proposed   &&          &        &         &          &        &          &        &         &            \\
                
                \cmidrule{1-1} \cmidrule{3-11}
                CFP-MD to UWF-MD\\
                \cmidrule{1-1} \cmidrule{3-11}
                Model-CFP   &&          &        &         &          &        &          &        &         &    \\
                Model-UWF   &&          &        &         &          &        &          &        &         &     \\
                Model-Transfer   &&          &        &         &          &        &          &        &         &     \\

                DDC\cite{DDC}   &&          &        &         &          &        &          &        &         &     \\
                DANN\cite{DANN}   &&          &        &         &          &        &          &        &         &       \\
                ADDA\cite{ADDA}   &&          &        &         &          &        &          &        &         &            \\
                MDD\cite{MDD}   &&          &        &         &          &        &          &        &         &            \\
                FixBi\cite{FixBi}   &&          &        &         &          &        &          &        &         &            \\
                CycleGan\cite{FixBi}   &&          &        &         &          &        &          &        &         &           \\
                Proposed   &&          &        &         &          &        &          &        &         &            \\
                
                \cmidrule{1-1} \cmidrule{3-11}
                RFMiD to TOP\\
                \cmidrule{1-1} \cmidrule{3-11}
                Model-CFP   &&          &        &         &          &        &          &        &         &    \\
                Model-UWF   &&          &        &         &          &        &          &        &         &     \\
                Model-Transfer   &&          &        &         &          &        &          &        &         &     \\

                DDC\cite{DDC}   &&          &        &         &          &        &          &        &         &     \\
                DANN\cite{DANN}   &&          &        &         &          &        &          &        &         &       \\
                ADDA\cite{ADDA}   &&          &        &         &          &        &          &        &         &            \\
                MDD\cite{MDD}   &&          &        &         &          &        &          &        &         &            \\
                FixBi\cite{FixBi}   &&          &        &         &          &        &          &        &         &            \\
                CycleGan\cite{FixBi}   &&          &        &         &          &        &          &        &         &           \\
                Proposed   &&          &        &         &          &        &          &        &         &            \\
            
            \end{tabular}
        }
    }
\end{table*}

==> table/sota-short.tex <==
\begin{table*}[htb]
    \caption{\textbf{Performances of different methods.}}
    \label{tab:sota-short}
    \centerline{
        \scalebox{0.5}{
            \begin{tabular}{ll rr  rr  r}
                \hline
                \textbf{Method} && \textbf{RFMiD$\rightarrow$TOP} && \textbf{CFP-MD$\rightarrow$CFP-UWF} && \textbf{CFP-MD$\rightarrow$CFP-WF}  \\
                \cmidrule{1-1} \cmidrule{3-3}  \cmidrule{5-5} \cmidrule{7-7}            
                Model-CFP           && 0.245$\pm$0.009 && 0.309$\pm$0.025 && 0.473$\pm$0.025 \\
                Model-UWF           && 0.647$\pm$0.036 && 0.622$\pm$0.018 && 0.669$\pm$0.003 \\
                Model-Transfer      && 0.640$\pm$0.018 && 0.623$\pm$0.005 && 0.680$\pm$0.018 \\

                DDC\cite{DDC}       && 0.624$\pm$0.015 && 0.652$\pm$0.006 && 0.675$\pm$0.002 \\
                DANN\cite{DANN}     && 0.628$\pm$0.006 && 0.640$\pm$0.013 && 0.686$\pm$0.006 \\
                ADDA\cite{ADDA}     && 0.663$\pm$0.022 && 0.617$\pm$0.012 && 0.679$\pm$0.007 \\
                MDD\cite{MDD}       && 0.644$\pm$0.012 && 0.640$\pm$0.015 && 0.678$\pm$0.007 \\
                FixBi\cite{FixBi}   && 0.653$\pm$0.024 && 0.635$\pm$0.011 && 0.652$\pm$0.015 \\
                CycleGAN\cite{ju2021leveraging} && 0.640$\pm$0.018 && 0.651$\pm$0.010 && 0.688$\pm$0.005 \\

                Proposed            && \textbf{0.678$\pm$0.032} && \textbf{0.675$\pm$0.009} && \textbf{0.691$\pm$0.006} \\
                \hline
            \end{tabular}
        }           
    }
\end{table*}

==> table/table_all.tex <==
\begin{table}[htb!]
    \caption{\textbf{Performance on different datasets}. For UWF-MD, WF-MD and TOP, the corresponding training data is CFP-MD + UWF-MD, CFP-MD + WF-MD and RFMiD + TOP, respectively.}
    \label{tab:uwf-all}
    \renewcommand{\arraystretch}{1.1}
    \centerline{
        \scalebox{0.65}{
            \begin{tabular}{@{}lrrrrrrrrr@{}}
        \toprule
                \textbf{Method} & \textbf{mAP} & \textbf{DR} &  \textbf{RVO} & \textbf{LP} & \textbf{DM} & \textbf{RD} & \textbf{TF} & \textbf{AMD} & \textbf{MEM}\\
                \midrule
                
                \textit{Supervised baselines:}\\
                \texttt{CFP} & 0.309$\pm$0.025 & 0.581 & 0.240 & 0.472 & 0.463 & 0.415 & 0.183 & 0.064 & 0.052 \\
                \texttt{UWF} & 0.622$\pm$0.018 & 0.726 & 0.498 & 0.927 & 0.868 & 0.840 & 0.620 & 0.340 & 0.161\\
                \texttt{UWF+} & 0.623$\pm$0.005 & 0.721 & 0.498 & 0.923 &0.883 & 0.843 & 0.611 & 0.309 & 0.198\\
                
                \midrule
                \textit{UDA baselines:}\\
                \texttt{ADDA} \cite{ADDA}  & 0.140$\pm$0.024 & 0.202 & 0.027 & 0.254 & 0.256 & 0.098 & 0.244 & 0.021 & 0.013\\
                \texttt{FixBi} \cite{FixBi} & 0.161$\pm$0.023 & 0.065 & 0.050 & 0.544 & 0.215 & 0.090 & 0.288 & 0.021 & 0.015\\
                \texttt{CDAN} \cite{CDAN} & 0.252$\pm$0.024 & 0.411 & 0.151 & 0.432 & 0.657 & 0.066 & 0.255 & 0.032 & 0.015\\
                \texttt{DDC} \cite{DDC} & 0.262$\pm$0.006 & 0.468 & 0.329 & 0.509 & 0.481 & 0.097 & 0.157 & 0.042 & 0.014\\ 
                \texttt{MDD} \cite{MDD} & 0.292$\pm$0.007 & 0.454 & 0.245 & 0.477 & 0.684 & 0.090 & 0.322 & 0.041 & 0.023\\
                \texttt{SDAT} \cite{SDAT} & 0.300$\pm$0.019 & 0.503 & 0.256 & 0.549 & 0.712 & 0.057 & 0.264 & 0.045 & 0.015\\
                \texttt{DANN} \cite{DANN} &  0.306$\pm$0.011 & 0.489 & 0.286 & 0.497 & 0.768 & 0.075 & 0.246 & 0.065 & 0.018\\
                \texttt{MIC} \cite{MIC} & 0.314$\pm$0.009 & 0.531 & 0.264 & 0.556 & 0.719 & 0.069 & 0.291 & 0.059 & 0.020\\  
                \texttt{ELS} \cite{ELS} & 0.318$\pm$0.007 & 0.584 & 0.235 & 0.544 & 0.735 & 0.066 & 0.300 & 0.064 & 0.017\\
                                
                \midrule
                \textit{SDA baselines:}\\
                \texttt{CDAN} \cite{CDAN} & 0.570$\pm$0.012 & 0.691 & 0.456 & 0.891 & 0.890 & 0.788 & 0.556 & 0.250 & 0.039\\
                \texttt{ADDA} \cite{ADDA}  & 0.617$\pm$0.012 & 0.726 & 0.467 & 0.923 & 0.883 & 0.825 & 0.590 & 0.306 & 0.220\\
                \texttt{FixBi} \cite{FixBi} & 0.635$\pm$0.011 & 0.710&0.486&0.912&0.888&\textbf{0.861}&0.594&0.422&0.204 \\
                \texttt{MDD} \cite{MDD} & 0.640$\pm$0.015 & 0.712&0.451&0.909&0.860&0.815&0.585&0.532&0.259\\
                \texttt{DANN} \cite{DANN} &  0.640$\pm$0.013 & 0.717&0.423&0.906&0.881&0.827&0.586&0.526&0.251\\
                \texttt{SDAT} \cite{SDAT} & 0.641$\pm$0.016 & 0.746 & 0.458 & 0.928 & 0.909 & 0.838 & 0.610 & 0.444 & 0.193\\
                \texttt{MIC} \cite{MIC} & 0.642$\pm$0.013 & 0.722 & 0.447 & 0.900 & 0.896 & 0.804 & 0.600 & 0.484 & 0.280\\   
                \texttt{CycleGAN} \cite{ju2021leveraging} & 0.651$\pm$0.010 & 0.679&0.471&0.923&0.890&0.817&0.579&0.518&0.331\\
                \texttt{DDC} \cite{DDC} & 0.652$\pm$0.006 & 0.689&0.433&0.888&0.879&0.825&0.616&0.467&\textbf{0.419}\\ 
                \texttt{ELS} \cite{ELS} & 0.656$\pm$0.007 & 0.741 & 0.469 & \textbf{0.934} & \textbf{0.913} & 0.848 & \textbf{0.628} & 0.457 & 0.262\\

                \midrule
                \textit{Proposed:} \\
                \texttt{CdCL} & \textbf{0.675}$\pm$0.009 & \textbf{0.747}&0.475&0.932&0.887&0.845&0.614&\textbf{0.581}&0.318\\
                \emph{w/o} CFP & 0.638$\pm$0.010 & 0.732&0.486&0.923&\textbf{0.896}&0.846&0.612&0.431&0.179\\
                \emph{w/o}  \texttt{SbC} & 0.645$\pm$0.026&0.720&0.503&0.920&0.887&0.835&0.615&0.409&0.273 \\
                \emph{w/o}  \texttt{GAP} & 0.662$\pm$0.007 & 0.723&\textbf{0.511}&0.906&0.883&0.832&0.608&0.498&0.331\\
        \bottomrule
            \end{tabular}
        }           
    }
    \vspace{-0.cm}
\end{table}
